Qiana: A First-Order Formalism to Quantify over Contexts and Formulas with Temporality

We introduce Qiana, a logic framework for reasoning on formulas that are true only in specific contexts. In Qiana, it is possible to quantify over both formulas and contexts to express, e.g., that ``everyone knows everything Alice says''. Qiana also permits paraconsistent logics within contexts, so that contexts can contain contradictions. Furthermore, Qiana is based on first-order logic, and is finitely axiomatizable, so that Qiana theories are compatible with pre-existing first-order logic theorem provers. We show how Qiana can be used to represent temporality, event calculus, and modal logic. We also discuss different design alternatives of Qiana.

==> Backups/Notations.tex <==
\SC{
    Please feel free to change the symbols used in these notations by updating the macros in the symbols.tex file. I used the $\bigcirc$ symbol because it is used for time in LTL and other temporal logics; but I am open to suggestions.
}
\FS{I do not understand the title of the section. "Bette rnotation". If the reader reads that, she thinks "why not having introduced beter notations right from the beginning then?" }

In order to simplify the writing of Qiana formulas, we introduce the following shorthand notations: \fms{As we briefly discussed, I personally think that this notation does not help much -- neither in terms of space, nor in terms of clarity. It might also add confusion with the later modal operators, and attract smirks when we also add the circles... So I would propose we reduce this notation to a remark somewhere.}

$$\context{c} t \equiv \ist(c,t)$$
$$\contextq{c} \varphi \equiv \ist(c, \bm \varphi)$$

The construction $\context{c} t$ is read as ``in $c$, $t$ holds'' and $\contextq{c} \varphi$ is read as ``in $c$ quote $\varphi$ holds''.

\FS{The previous notations could be moved after "ist".}

\FS{The following notations for temporal reasoning should be in the section "Temporality in Qiana"? Then this section disappears :). Again it is normal that notations about time are defined in the section about time! The reader expects that. Always minimize the surprise!}\fms{agreed}

\SC{It is weird to include this remark here. Originally, it was in the discussion section. But the other part of the section is now obsolete (it was discussing types, which we since added to the article.)
I decided it was weird to have an entire section just for this remark.
The natural place for this remark would be right after the definition of Qiana, but I do not want people to read it before they have built a better intuition through the example section.
I put it here because this section is small and because it is sufficiently late in the article, even though it feels a bit disconnected from the rest of the section.}
\FS{No the remark should be after the definition of Qiana. The remark should be where the reader expects it to be. Otherwise, the article is not well-structured. }\fms{agreed. Especially if the remark is called ``on the definition of V'' :-)}

==> Backups/Time.tex <==
In this sections we extend Qiana for temporal reasoning.
We do so by adapting the axioms of event calculus to Qiana. 

\subsection{Overview of Event Calculus}
\SC{Explain more event calculus?}
Event calculus is one of the most popular formalisms to represent actions and their effects on systems through time.
In this article, we follow the definitions of~\citeA{EventCalculusExplained} \fms{again, justify}. This calculus is based on the following concepts:
\textit{Fluents} are properties of the system that can change over time. There is typically a finite set of fluent under consideration.
\textit{Actions} (also called \textit{Events}) occur at point in time or during time intervals and can change the value of fluents.
\fms{ok, what's the difference between actions and events?} \SCI{For our purposes, none. Per my understanding the distinction is useful in formalisms that want to model agents and their actions as special, hence the existence of two terms. I hesitated to remove the word ``event'' altogether; but that would be weird given the name of the calculus.}

\fms{We might need a definition of the main event calculus operators. We might also need a formal definition, without which it will be difficult to stage proofs...} Here are a few example sentences written in classical event calculus and toying with the Romeo and Juliet story:
    $$\textit{HoldsAt}(\textit{Alive\_Romeo},i)$$
This means that Romeo is alive at instant $i$. Here the fluent is $\textit{Alive\_Romeo}$ and the time is $i$.
    $$\textit{Happens}(\textit{Drink\_Potion\_Juliet},i)$$
\fms{could these examples be chosen so as to show the specific capacities of the calculus? In particular, can Juliet die in this calculus? Also, do we have only propositional logic in this system?}
\SCI{There is no logic on fluents, propositional or otherwise.}
This means that Juliet drinks a potion at time $i$. Here the action is $\textit{Drink\_Potion\_Juliet}$.
    $$\textit{Happens}(\textit{Drink\_Potion\_Juliet},i_1,i_2)$$
This means that Juliet drinks a potion between time $i_1$ and $i_2$. Here the action is $\textit{Drink\_Potion\_Juliet}$. Note the operator overload on $\textit{Happens}$ with the previous statement. The same can be done with $\textit{HoldsAt}$.
    $$\textit{Initiates}(\textit{Appear\_Dead\_Juliet},\textit{Drink\_Potion\_Juliet},i)$$
This means that drinking a potion makes Juliet start appearing dead at time $i$. Here the fluent is $\textit{Appear\_Dead\_Juliet}$ and the action is $\textit{Drink\_Potion\_Juliet}$.

This concludes our limited presentation of event calculus.
In the next subsection we will present the Qiana version of these operators and of other useful temporal operators.

% % SIMON : I simplified the remark and removed references to the frame problem.
% \begin{remark}[A word on the frame problem]
%     We summarize the frame problem as follows: ``Most of the time things do not change if nothing makes them change. This is inertia: the tendency for systems to remain in their current state. How can we write formalisms that capture this without writting rules to list exhaustively all the situations that permit something to change?''
%     In event calculs, the solution comes in part from the semantics, which is nonmonotonic: under some circumstances we assume things remain the same unless proven otherwise.
%     We cannot port this semantic to Qiana directly, which means we will need to write more complexe rules and indeed list exhaustively the conditions under which something changes.
% \end{remark}


\subsection{Event calculus in Qiana}

We will now show how the event calculus of \citeA{EventCalculusExplained} can be mirrored in Qiana. The event calculus of \citeA{EventCalculusExplained} comes both with its own axiomatization and with a semantic. In this section we copy the behavior of this calculus by adapting the axioms to Qiana but we do not introduce a new semantics. We do, however, show how to broaden the calculus of \citeA{EventCalculusExplained} from purely propositional fluents to first-order with quantifiers.
    
We introduce temporality to Qiana with Axiom~\ref{ax:ECQ1} to Axiom~\ref{ax:ECQlast}, which are adapted from the ones of the ``full event calculus'' as described in~\citeA{EventCalculusExplained}.
The main difference is that Qiana permits the use of any well formed closed quoted formula in place of fluents, strongly broadening the scope of temporal statements.

\noindent We also introduce the following notations to help us write temporal statements more concisely:
$$\timeIns{i_1} t \equiv \ist(\textit{at}(i_1), t)$$
$$\timeSpan{i_1}{i_2} t \equiv \ist(\textit{between}(i_1, i_2), t)$$

The construction $\timeIns{i_1} t$ is read as ``at $i_1$, $t$ holds'' and $\timeSpan{i_1}{i_2} t$ is read as ``between $i_1$ and $i_2$, $t$ holds''.
$\textit{at}(i_1)$ and $\textit{between}(i_1, i_2)$ define temporal contexts (which are distinct from time instants $i_1$ and $i_2$). Our equivalents to the event calculus operators are statements within these contexts.
\SC{
    A discussion to be had: 
    Do we allow temporal statements to be used as fluents? It seems to make no sense. 
    This leads to a discussion on introduced types, to be had offline.
}\fms{how about we say in the discussion of typing: loom, typing can avoid this particular oddity of fluents inside fluents. I don't think the question will appear in the present section :-) }

We present in Table~\ref{table:ECopsInQiana} and Table~\ref{table:ECopsToQian} the Qiana notations for the event calculus operators. 

\begin{table}[h!]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    Qiana notation & Description  \\ 
    \hline
    0 & The first time instant \\
    $i_1 < i_2$ & Instant $i_1$ occurs before instant $i_2$ \\
    $\textit{Initially}(\bm \varphi)$ & Nontemporal quoted formula $\bm \varphi$ holds at the beginning \\
    $\timeIns{i_1} \bm \varphi$ & Nontemporal quoted formula $\bm \varphi$ holds at time $i_1$ \\ 
    $\timeSpan{i_1}{i_2} \bm \varphi$ & $\bm \varphi$ holds between times $i_1$ and $i_2$ \\ 
    $\timeIns{i_1} \textit{Happens}(a)$  & Action $a$ happens at time $i_1$ \\
    $ \timeIns{i_1} \textit{Initiates}(a, \bm \varphi)$ & If action occurs at time $i_1$ it initiates $\bm \varphi$ at that time \\
    $ \timeIns{i_1} \textit{Terminates}(a, \bm \varphi)$ &  If action occurs at time $i_1$ it terminates $\bm \varphi$ at that time \\
    $ \timeIns{i_1} \textit{Releases}(a, \bm \varphi)$ & $\bm \varphi$ is not subject to inertia after action $a$ at time $i_1$ \\
    $ \timeSpan{i_1}{t_2} \textit{Clipped}(\bm \varphi)$ & $\bm \varphi$ is terminated between times $i_1$ and $i_2$ \\
    $ \timeSpan{i_1}{t_2} \textit{Declipped}(\bm \varphi)$ & $\bm \varphi$ is initiated between times $i_1$ and $i_2$ \\
    \hline
    \end{tabular}
    \caption{Description of Qiana temporal operators} \label{table:ECopsInQiana}
\end{table}




\begin{table}[h!]
    \centering
    \begin{tabular}{|c|c|}
    \hline
    Qiana notation & Event Calculus operator \\ 
    \hline
    0 &  0\\
    $i_1 < i_2$ & $i_1 < i_2$\\
    $\textit{Initially}(\bm \varphi)$ & $\textit{Initially}(\bm \varphi)$\\
    $\timeIns{i_1} \bm \varphi$ & $\textit{HoldsAt}(i_1,\bm \varphi)$\\ 
    $\timeSpan{i_1}{i_2} \bm \varphi$ & $\textit{HoldsAt}(i_1, i_2,\bm \varphi)$\\ 
    $\timeIns{i_1} \textit{Happens}(a)$ & $\textit{Happens}(a, i_1)$\\
    $ \timeIns{i_1} \textit{Initiates}(a, \bm \varphi)$ & $\textit{Initiates}(a, \bm \varphi, i_1)$\\
    $ \timeIns{i_1} \textit{Terminates}(a, \bm \varphi)$ & $\textit{Terminates}(a, \bm \varphi, i_1)$\\
    $ \timeIns{i_1} \textit{Releases}(a, \bm \varphi)$ &  $\textit{Releases}(a, \bm \varphi, i_1)$\\
    $ \timeSpan{i_1}{t_2} \textit{Clipped}(\bm \varphi)$ & $\textit{Clipped}(i_1, \bm \varphi, i_2)$\\
    $ \timeSpan{i_1}{t_2} \textit{Declipped}(\bm \varphi)$ & $\textit{Declipped}(i_1, \bm \varphi, i_2)$\\
    \hline
    \end{tabular}
    \caption{Matching Qiana notation to event calculus operators} \label{table:ECopsToQian}
\end{table}



\begin{table}[h!]
    \centering
    \scalebox{0.9}{
    \begin{tabular}{|c|c|l|} % modify the last l into p{6cm} if you prefer having the description on several lines
    \hline
    Qiana notation & Event Calculus operator & Description \\ 
    \hline
    0 &  0 & The first time instant \\
    $i_1 < i_2$ & $i_1 < i_2$ & Instant $i_1$ occurs before instant $i_2$ \\
    $\textit{Initially}(\bm \varphi)$ & $\textit{Initially}(\bm \varphi)$ & Nontemporal quoted formula $\bm \varphi$ holds at the beginning \\
    $\timeIns{i_1} \bm \varphi$ & $\textit{HoldsAt}(i_1,\bm \varphi)$
    & Nontemporal quoted formula $\bm \varphi$ holds at time $i_1$
    \\ 
    $\timeSpan{i_1}{i_2} \bm \varphi$ & $\textit{HoldsAt}(i_1, i_2,\bm \varphi)$ 
    & $\bm \varphi$ holds between times $i_1$ and $i_2$
    \\ 
    $\timeIns{i_1} \textit{Happens}(a)$ & $\textit{Happens}(a, i_1)$
    & Action $a$ happens at time $i_1$
    \\
    $ \timeIns{i_1} \textit{Initiates}(a, \bm \varphi)$ & $\textit{Initiates}(a, \bm \varphi, i_1)$ 
    & 
    If action occurs at time $i_1$ it initiates $\bm \varphi$ at that time 
    \\
    $ \timeIns{i_1} \textit{Terminates}(a, \bm \varphi)$ & $\textit{Terminates}(a, \bm \varphi, i_1)$ &  If action occurs at time $i_1$ it terminates $\bm \varphi$ at that time \\
    $ \timeIns{i_1} \textit{Releases}(a, \bm \varphi)$ &  $\textit{Releases}(a, \bm \varphi, i_1)$ & $\bm \varphi$ is not subject to inertia after action $a$ at time $i_1$ \\
    $ \timeSpan{i_1}{t_2} \textit{Clipped}(\bm \varphi)$ & $\textit{Clipped}(i_1, \bm \varphi, i_2)$& $\bm \varphi$ is terminated between times $i_1$ and $i_2$ \\
    $ \timeSpan{i_1}{t_2} \textit{Declipped}(\bm \varphi)$ & $\textit{Declipped}(i_1, \bm \varphi, i_2)$& $\bm \varphi$ is initiated between times $i_1$ and $i_2$ \\
    \hline
    \end{tabular}}
    \caption{Matching Qiana notation to event calculus operators} \label{table:ECopsToQian}
\end{table}

\SC{I split this table in two, I couldn't make it fit otherwise.}
\FS{I succeeded. Do you like? I think it is better to have ONE table!}
\SC{I did not include initiallyN, we can just do Initially$\neg$}

% \begin{align}
%     & \forall f, i.\ \timeIns{i} f \leftarrow \textit{Initially(}(f) \land \neg \timeSpan{0}{i} \textit{Clipped}(f) \label{ax:ECQ1} \\
%     & \forall f, a, i_1, i_2, i_3.\ \timeIns{i_3}f \leftarrow \timeSpan{i_1}{i_2}\textit{Happens}(a) \land \timeIns{i_1} \textit{Initiates}(a,f) \land i_2 < i_3  
%         \nonumber \\ &\hspace{8cm} \land \neg \timeSpan{i_1}{i_3} \textit{Clipped}(f) \\
%     & \forall f, a, i_1, i_4.\ \timeSpan{i_1}{i_4} \textit{Clipped}(f) \leftrightarrow ( \exists a,i_2,i_3.\ \timeSpan{i_2}{i_3} \textit{Happens}(a) \land i_1 < i_3 \land i_2 < i_4 
%         \nonumber \\ &\hspace{6cm} \land (\timeIns{i_2} \textit{Terminates}(a,f) \lor \timeIns{i_2} \textit{Releases}(a,f))) \\
%     & \forall O, f, i.\ \neg \timeIns{i} f \leftarrow \textit{Initially(}(\bneg\ f) \land \neg \timeSpan{0}{i} \textit{Declipped}(f) \\
%     & \forall f, a, i_1, i_2, i_3.\ \timeIns{i_3} f \leftarrow \timeSpan{i_1}{i_3} \textit{Happens}(a) \land \timeIns{i_1} \textit{Terminates}(a,f) \land i_2 < i_3 
%         \nonumber \\ &\hspace{6cm} \land \timeSpan{i_1}{i_3} \textit{Declipped}(f) \\
%     & \forall f, a, i_1, i_2, i_3, i_4.\ \timeSpan{i_1}{i_4} \textit{Declipped}(f) \leftrightarrow (\exists a,i_2,i_3 (\timeSpan{i_2}{i_3} \textit{Happens}(a) \land i_1 < i_3 
%         \nonumber \\ &\hspace{5cm} \land i_2 < i_4 \land (\timeIns{i_2} \textit{Initiates}(a,f) \lor \timeIns{i_2} \textit{Releases}(a,f)))) \\
%     & \forall a, i_1, i_2.\ \timeSpan{i_1}{i_2} \textit{Happens}(a) \rightarrow i_1 \leq i_2 \label{ax:ECQlast}
% \end{align}

These operators are axiomatized as follows:

\begin{align}
    &\forall f, t .\ \textit{HoldsAt}(f, t) \leftarrow \textit{Initially}_P(f) \land \neg \textit{Clipped}(0, f, t)\tag{EC1} \\
    &\forall f, t_3, a, t_1, t_2 .\ \textit{HoldsAt}(f, t_3) \notag \\ & \hspace*{1cm} \leftarrow \textit{Happens}(a, t_1, t_2) \land \textit{Initiates}(a, f, t_1) \land t_2 < t_3 \land \neg \textit{Clipped}(t_1, f, t_3)\tag{EC2} \\
    &\forall t_1, f, t_4 .\ \textit{Clipped}(t_1, f, t_4) \leftrightarrow \exists a, t_2, t_3 .\ \textit{Happens}(a, t_2, t_3) \land t_1 < t_3 \land t_2 < t_4 \land \notag \\ &\hspace*{1cm} (\textit{Terminates}(a, f, t_2) \lor \textit{Releases}(a, f, t_2))\tag{EC3} \\
    &\forall f, t .\ \neg \textit{HoldsAt}(f, t) \leftarrow \textit{Initially}_N(f) \land \neg \textit{Declipped}(0, f, t)\tag{EC4} \\
    &\forall f, t_3, a, t_1, t_2 .\ \neg \textit{HoldsAt}(f, t_3) \notag \\ & \hspace*{1cm} \leftarrow \textit{Happens}(a, t_1, t_2) \land \textit{Terminates}(a, f, t_1) \land t_2 < t_3 \land \neg \textit{Declipped}(t_1, f, t_3)\tag{EC5} \\
    &\forall t_1, f, t_4 .\ \textit{Declipped}(t_1, f, t_4) \leftrightarrow \exists a, t_2, t_3 .\ \textit{Happens}(a, t_2, t_3) \land t_1 < t_3 \land t_2 < t_4 \land \notag \\
    &\hspace*{1cm} (\textit{Initiates}(a, f, t_2) \lor \textit{Releases}(a, f, t_2))\tag{EC6} \\
    &\forall a, t_1, t_2 .\ \textit{Happens}(a, t_1, t_2) \rightarrow t_1 \leq t_2\tag{EC7}
\end{align}

\begin{align}
    & \forall f, i.\ \textit{Initially}(f) \land \neg \timeSpan{0}{i} \textit{Clipped}(f) \rightarrow \timeIns{i} f \label{ax:ECQ1} \\
    & \forall f, a, i_1, i_2, i_3.\ \timeSpan{i_1}{i_2}\textit{Happens}(a) \land \timeIns{i_1} \textit{Initiates}(a,f) \land i_2 {<} i_3 \land \neg \timeSpan{i_1}{i_3} \textit{Clipped}(f) \\ & \nonumber \hspace{6cm} \rightarrow \timeIns{i_3}f \\
    & \forall f, a, i_1, i_4.\ \timeSpan{i_1}{i_4} \textit{Clipped}(f) \leftrightarrow  \\ & \nonumber \exists a,i_2,i_3.\ \timeSpan{i_2}{i_3} \textit{Happens}(a) \land i_1 {<} i_3 \land i_2 {<} i_4 \land (\timeIns{i_2} \textit{Terminates}(a,f) \lor \timeIns{i_2} \textit{Releases}(a,f)) \\
    & \forall O, f, i.\ \textit{Initially}(\bneg\ f) \land \neg \timeSpan{0}{i} \textit{Declipped}(f) \rightarrow \neg \timeIns{i} f \\
    & \forall f, a, i_1, i_2, i_3.\ \timeSpan{i_1}{i_3} \textit{Happens}(a) \land \timeIns{i_1} \textit{Terminates}(a,f) \land i_2 {<} i_3 \land \timeSpan{i_1}{i_3} \textit{Declipped}(f) \nonumber \\ &\hspace{6cm} \rightarrow \timeIns{i_3} f \\
    & \forall f, a, i_1, i_2, i_3, i_4.\ \timeSpan{i_1}{i_4} \textit{Declipped}(f) \leftrightarrow \\ & \nonumber (\exists a,i_2,i_3 (\timeSpan{i_2}{i_3} \textit{Happens}(a) \land i_1 {<} i_3 
         \land i_2 {<} i_4 \land (\timeIns{i_2} \textit{Initiates}(a,f) \lor \timeIns{i_2} \textit{Releases}(a,f)))) \\
    & \forall a, i_1, i_2.\ \timeSpan{i_1}{i_2} \textit{Happens}(a) \rightarrow i_1 {\leq} i_2 \label{ax:ECQlast}
\end{align}
\SC{I struggled quite a bit to make the axioms prettier. If you think you can do better, please feel free.}
\FS{I put reduce the space around $<$ and $\leq$}
When a formula is initiated it becomes true and gains inertia by default.
This means it will remain true unless it is clipped, as stated in Axiom~\ref{ax:ECQ1}.

\subsection{Example}

We will now adapt our running example of Romeo and Juliet (Section~\ref{subsec:suicideExample}) to our temporal framework.
We will tell the same story as before but we will now account for time:
%contrary to what we did in Section~\ref{sec:Example}.
At first Romeo is alive, then he sees Juliet, then he dies. We will use the following axioms:
\begin{align}
    & \forall \varphi.\ \ist(\textit{says}(\textit{L}), \varphi) \rightarrow \truth(\varphi) \label{ex:EC_RJ1}\\
    & \ist(\textit{says(\textit{L})},  \fquo{\forall i.\ \timeIns{i} \textit{Happens}(\textit{drink}(P,J))}) \rightarrow \timeIns{i} \textit{Initiate}(\textit{drink}(J,P), \bm{\textit{LookDead}}(J)) \label{ex:EC_RJ2}\\
    & t_\textit{drink} < t_\textit{see} \label{ex:EC_RJ8}\\
    & \timeIns{t_\textit{drink}} \textit{Happens}(\textit{drink}(P,J)) \label{ex:EC_RJ3}\\
    & \timeIns{t_\textit{see}} \textit{Happens}(\textit{see}(R,J)) \label{ex:EC_RJ6} \\
    & \neg \timeSpan{t_\textit{dringk}}{t_\textit{see}} \textit{Clipped}(\textit{LookDead}(J)) \label{ex:EC_RJ4}\\
    & \forall i_1, p, i_2.\ \timeIns{i_1}  \bm{\textit{LookDead}}(\quot(p)) \rightarrow \timeIns{i_1} \textit{Initiate}(\textit{See}(R,p), \bm{\ist(\textit{bel}(R), \bm{dead(p)})}) \label{ex:EC_RJ5} \\
    & \forall i_1. \timeIns{i_1} \ist(\textit{bel}(R), \fquo{dead(J)}) \rightarrow \timeIns{i_1} \textit{Happens}(\textit{die}(R)) \label{ex:EC_RJ7}
\end{align}

Note the different elements:
$\textit{See}(R,J)$ is an action, just like $\textit{die}(R)$.
$\textit{LookDead}(J)$ is a formula (like $\textit{dead}(J)$), its quotation is a fluent. Two points in time are important to the story: the time $t_\textit{drink}$ when Juliet drinks the potion and the time $t_\textit{see}$ when Romeo sees Juliet. 
Formulas~\ref{ex:EC_RJ1} and~\ref{ex:EC_RJ2} behave similarly to their counterparts in Section~\ref{subsec:suicideExample}, except that Laurence now says Juliet will ``start looking dead'', rather than simply ``look dead''.
Formula~\ref{ex:EC_RJ3} states that Juliet drinks the potion, and formula~\ref{ex:EC_RJ4} states that Juliet does not wake up before $t_\textit{see}$.
Hence Juliet looks dead at time $t_\textit{see}$.
Together with formulas~\ref{ex:EC_RJ6} and~\ref{ex:EC_RJ5} this tells us that Romeo starts believing Juliet is dead, which leads to his own death (Formula~\ref{ex:EC_RJ7}).

\fms{This example could be strengthened significantly if we could formulate it in Qiana, translate it to TPTP, run it in Vampire, and report the result here. This may sound like a lot of effort but it would allow us to check that everything works indeed as intended. }

